Implicit Knowledge in Argumentative Texts: An Annotated Corpus

When speaking or writing, people omit information that seems clear and evident, such that only part of the message is expressed in words. Especially in argumentative texts it is very common that (important) parts of the argument are implied and omitted. We hypothesize that for argument analysis it will be beneficial to reconstruct this implied information. As a starting point for filling such knowledge gaps, we build a corpus consisting of high-quality human annotations of missing and implied information in argumentative texts. To learn more about the characteristics of both the argumentative texts and the added information, we further annotate the data with semantic clause types and commonsense knowledge relations. The outcome of our work is a carefully de-signed and richly annotated dataset, for which we then provide an in-depth analysis by investigating characteristic distributions and correlations of the assigned labels. We reveal interesting patterns and intersections between the annotation categories and properties of our dataset, which enable insights into the characteristics of both argumentative texts and implicit knowledge in terms of structural features and semantic information. The results of our analysis can help to assist automated argument analysis and can guide the process of revealing implicit information in argumentative texts automatically.

==> 5.4.tex <==
\subsection{Co-Occurrences of Commonsense Relation Types} Finally, we want to learn more about the properties of the texts in our dataset in terms of co-occurrences of commonsense relation types. We distinguish between relations labelled for each microtext (Fig.\ \ref{fig:cooc}, left) and relations labelled for each set of inserted sentences (Fig.\ \ref{fig:cooc}, right). 

 Our symmetric heatmap shows that %\orangenote{
\textsc{CapableOf} occurs often more than once in the same microtext (that means that in the same text, \textsc{CapableOf} is used several times), the same we observe for \textsc{HasProperty}. Other frequently co-occurring relations within the microtexts are for example \textsc{HasPrerequisite} and \textsc{HasProperty}, \textsc{CapableOf} and \textsc{Causes}, and \textsc{CapableOf} and \textsc{UsedFor}.

Fig.\ \ref{fig:cooc} (right side) shows that the relations \textsc{CapableOf}, \textsc{HasProperty}, and \textsc{Causes} occur often more than once % \orangenote{more than once? this is a correlation value. Do you rather want to say that they co-occur/correlate with more than one other relation type?}
within the same set of inserted information. Furthermore, the relations \textsc{Causes} and \textsc{CapableOf}, and \textsc{CapableOf} and \textsc{HasA} co-occur most frequently together within the sets of inserted sentences. We interpret these observed co-occurrences of specific commonsense relation types %are more frequent then others and could therefore be interpreted 
as features of argumentative texts/of implicit knowledge annotations, that can be used for characterizing and distinguishing these text types. 

\begin{figure*}[t]
\begin{centering}
\includegraphics[width=0.8
\textwidth]{figures/cooc-microtexts-setinserted.png}
\caption{Co-occurences of Commonsense Relations within each microtext (left) vs. each set of inserted sentences per argument unit pair (right), relative frequency.}
\vspace{0.3cm}
\label{fig:cooc}
\end{centering}
\end{figure*}

==> researchquestions.tex <==
Analyse correlations between...
\begin{itemize}
\itemsep-5pt
\item relation types
\item SE types
\item number of inserted sentences (hops)
\item argumentative relatedness
\item argumentative function
\item adjacency of units
\item …?
\end{itemize}


Interesting correlations might be between...
\begin{itemize}
\itemsep-5pt
\item argumentative relation and commonsense relations of inserted sentences
\item argumentative relation and clause type of inserted sentences
\item adjacency and commonsense relations of inserted sentences
\item adjacency and clause type of inserted sentences
\item commonsense relation and clause type
\item …?
\end{itemize}

Interesting research questions:
\begin{itemize}
\itemsep-5pt
\item Do specific semantic clause types appear more often in single (one inserted sentence) vs. multiple hops (more than one inserted sentence)?
\item Do specific commonsense relation types appear more often in single (one inserted sentence) vs. multiple hops (more than one inserted sentence)?
\item Do we find specific co-occurrences of commonsense relation types?
\item Do multiple hops correlate with non-adjacency?
\item In case of multiple hops for non-adjacent pairs: do arguments that occur in the intermediate relations also occur in the text that lies in-between pairs?
\item Do multiple hops correlate with a specific distribution of situation entity types?
\item Do we find more implicit statements in the beginning vs. the end of arguments? (works only for adjacent pairs)
\item …?
\end{itemize}
